Skeletal filtrations of the fundamental group of a non-archimedean curve

In this paper we study skeleta of residually tame coverings of a marked curve over a non-archimedean field. We first generalize a result by Liu and Lorenzini by proving a simultaneous semistable reduction theorem for residually tame coverings. We then use this to construct a functor from the category of residually tame coverings of a marked curve $(X,D)$ to the category of tame coverings of a metrized complex $\Sigma$ associated to $(X,D)$. We enhance the latter category by adding a set of gluing data to every covering and we show that this yields an equivalence of categories. Using this equivalence, we then define filtrations of the fundamental group of the marked curve, giving for instance the absolute decomposition and inertia groups of the metrized complex. We then use the analytic slope formula to prove that the extensions that arise from the abelianizations of the decomposition and inertia quotients coincide with the extensions that arise from the toric and connected parts of the analytic Jacobian of the curve.

==> AnalyticPreliminaries.tex <==
\subsection{Analytic preliminaries}\label{AnalyticPreliminaries}

We will now quickly review the various analytic notions we will be needing in this paper. For any $K$-algebra $A$, we denote its Berkovich spectrum by $\mathcal{M}(A)$. That is, it is the set of all bounded multiplicative seminorms on $A$ and we give it the weakest topology such that all real-valued functions of the form $|\,|\mapsto{|f|}$ are continuous for all $f\in{A}$. An {\it{analytic curve}} will be a strictly $K$-analytic space $Y$ of dimension $1$. For every algebraic curve $X$, there is a canonical analytic curve $X^{\mathrm{an}}$ associated to it, which is also referred to as the analytification of $X$.
For any finite map $\phi:X'\rightarrow{X}$ of algebraic curves over $K$, we then also obtain from the Berkovich analytification functor a finite map of analytic spaces $\phi^{\mathrm{an}}:X'^{\mathrm{an}}\rightarrow{X^{\mathrm{an}}}$. We will say that $\phi$ is {\it{tame}} if $\phi^{\mathrm{an}}$ is topologically tame in the sense of \cite[Section 3.2.3]{Cohen2016} and \cite[Section 6.3]{Berkovich1993}. That is, $\phi^{\mathrm{an}}$ is topologically tame if the local degrees $[\mathcal{H}(x'):\mathcal{H}(x)]$ are invertible in $k$ for all points $x'\in{X'^{\mathrm{an}}}$ mapping to $x\in{X^{\mathrm{an}}}$. Here $\mathcal{H}(x)$ is the completed residue field of a point in $X^{\mathrm{an}}$. %basic analytic domains connected to these curves. %affinoid domains These analytic curves are covered by affinoid domains, which we will quickly review. % and we will give a quick review 
%\subsubsection{Analytic building blocks}\label{BuildingBlocks}

Let $\mathbf{A}_{1}^{\mathrm{an}}:=\mathcal{M}(K[T])$ be the analytic affine line. We define the tropicalization map $\mathrm{trop}:\mathbf{A}_{1}^{\mathrm{an}}\rightarrow{\mathbb{R}\cup\{\infty\}}$ by
\begin{equation}
\mathrm{trop}(||\cdot{}||)=-\mathrm{log}(||T||).
\end{equation}
We will use this map to define the various analytic domains that we will be needing. We will be following  \cite[Section 2.1]{BPRa1}.

\begin{itemize}
\item Let $\mathbf{G}_{m}^{\mathrm{an}}=\mathcal{M}(K[T,1/T])$. Then $\mathbf{G}_{m}^{\mathrm{an}}=\mathrm{trop}^{-1}(\mathbb{R})$. 
\item Let $a\in{K^{*}}$. The standard closed ball of radius $|a|$ is $\mathbf{B}(a)=\mathrm{trop}^{-1}([\mathrm{val}(a),\infty])$. Its ring of analytic functions is then denoted by $K\langle{a^{-1}t}\rangle$, with canonical reduction $k[\tau]$, where $\tau$ is the residue of $a^{-1}t$.
\item Let $a\in{K^{*}}$. We define the standard open ball of radius $|a|$ to be $\mathbf{B}(a)_{+}=\mathrm{trop}^{-1}((\mathrm{val}(a),\infty))$. It can be written as an increasing union of standard closed balls.
\item Let $a,b\in{K^{*}}$ with $|a|\leq{|b|}$. The standard closed annulus of inner radius $|a|$ and outer radius $|b|$ is $\mathbf{S}(a,b)=\mathrm{trop}^{-1}([\mathrm{val}(a),\mathrm{val}(b)])$. Its ring of analytic functions is denoted by $K\langle{at^{-1},b^{-1}t}\rangle{}$. Its canonical reduction is then given by $k[\sigma,\tau]/(\sigma\tau-\overline{a/b})$, where $\sigma$ (resp. $\tau$) is the residue of $at^{-1}$ (resp. $b^{-1}t$) and $\overline{a/b}\in{k}$ is the residue of $a/b$. We define the length or modulus of $\mathbf{S}(a,b)$ to be $\mathrm{val}(a)-\mathrm{val}(b)$. 
\item In the situation above, if $|a|\leq{1}$ and $|b|=1$, we will denote the annulus by $\mathbf{S}(a):=\mathbf{S}(a,1)$. 
\item For $a,b\in{K^{*}}$ with $|a|<|b|$, we define the standard open annulus of inner radius $|a|$ and outer radius $|b|$ to be $\mathbf{S}(a,b)_{+}=\mathrm{trop}^{-1}((\mathrm{val}(b),\mathrm{val}(a)))$. This open analytic domain can again be expressed as an increasing union of standard closed annuli, see Equation (\ref{IncreasingUnion}) for an explicit description.
\item For $a\in{K}^{*}$, the standard punctured open ball of radius $|a|$ is $\mathbf{S}(0,a)_{+}=\mathrm{trop}^{-1}((\mathrm{val}(a),\infty))$. If $a=1$, we will write $\mathbf{S}(0)_{+}:=\mathbf{S}(0,1)_{+}$. 
\end{itemize}

We now define the tropicalization map on a torus. Let $A$ be a lattice of rank $n$, i.e. $A\simeq{\mathbb{Z}^{n}}$, let $B:=\mathrm{Hom}(A,\mathbb{Z})$ be the dual lattice and let $K[A]$ be the group ring corresponding to $A$. This is also called the character group of $A$. For $u\in{A}$, we write $\chi^{u}$ for the corresponding character in $K[A]$.
 We will write $A_{\mathbb{R}}:=A\otimes{\mathbb{R}}$ and $B_{\mathbb{R}}:=B\otimes{\mathbb{R}}$ for the corresponding real lattices. The torus with character lattice $A$ is then defined to be $T^{\mathrm{an}}:=\mathcal{M}(K[A])$, where $\mathcal{M}(\cdot{})$ denotes the Berkovich spectrum as defined in []. We define the {\it{tropicalization map}} $\mathrm{trop}:T^{\mathrm{an}}\rightarrow{B_{\mathbb{R}}}$ by 
\begin{equation}
(\mathrm{trop}(||\cdot{}||),u)=-\mathrm{log}(||\chi^{u}||). 
\end{equation} 
We then define the {\it{affinoid torus}} to be $T_{0}:=\mathrm{trop}^{-1}(0)$. We will see more of these tropicalizations of tori in Section \ref{Abelianization1}.



\subsection{Metrized complexes and harmonic morphisms}

In this section, we slightly expand upon several notions from \cite{ABBR1} to include disconnected metrized complexes and coverings thereof. The main reason we want to allow disconnected coverings is that we want our category to have coproducts, as in the algebraic case. The algebraic example we have in mind here is the %want to mimic here is the 
\'{e}tale covering $\mathrm{Spec}(\mathbb{C})\rightarrow{\mathrm{Spec}(\mathbb{R})}$, which splits into two disjoint schemes after taking the fiber product over the same morphism. %We fix a nontrivial subgroup $\Lambda$ of $(\mathbb{R},+)$ throughout this section.

We now generalize the notions of metric graphs, metrized complexes and harmonic morphisms to the disconnected case. 

%We start with reproducing some of the definitions in \cite{ABBR1}.
\begin{mydef}{\it{(Disconnected metric graphs)}}\label{MetricGraphsVertexSets}
A {\it{metric graph}} $\Gamma$ is a finite topological graph such that its connected components are metric graphs in the sense of \cite[Definition 2.2]{ABBR1}. We similarly define $\Lambda$-metric graphs and $\Lambda$-points. Here $\Lambda$ is the value group of the valuation on $K$. 

A {\it{vertex set}} $V(\Gamma)$ is a finite subset of the $\Lambda$-points of $\Gamma$ containing all essential vertices, as defined in \cite{ABBR1}. The edges of $\Gamma$ are the edges of the connected components $\Gamma_{i}$ of $\Gamma$. We will denote the induced vertex sets of the connected components $\Gamma_{i}$ by $V(\Gamma_{i})$. The induced edge sets are denoted by $E(\Gamma_{i})$. 
\end{mydef}

We now define morphisms of $\Lambda$-metric graphs. Let $\phi:\Gamma'\rightarrow{\Gamma}$ be a {\it{surjective}} continuous map of $\Lambda$-metric graphs. Since the image of a connected subset is again connected, we have induced surjective maps
\begin{equation}\label{MapsComponents1}
\phi_{i,j}:\Gamma'_{i,j}\rightarrow{\Gamma_{i}},
\end{equation}
where the $\Gamma_{i}$ are the connected components of $\Gamma$ and the $\Gamma'_{i,j}$ are the connected components of $\Gamma'$ mapping to $\Gamma_{i}$. For the remainder of the paper, we will label the maps on the connected components as above.  %We have chosen the labeling such that%$\Gamma'_{i,j}$ is any connected component of $\Gamma'$ and $\Gamma_{i}$ is the connected component of $\Gamma$ such that $\phi(\Gamma'_{i})\subset{\Gamma_{i}}$. Note that we can have $\Gamma_{i}=\Gamma_{j}$ for $i\neq{j}$. 
\begin{mydef} {\it{(Harmonic morphisms of disconnected metric graphs)}}\label{MorphismMetricGraph1}
Fix vertex sets $V(\Gamma')$ and $V(\Gamma)$ for two (possibly disconnected) $\Lambda$-metric graphs $\Gamma'$ and $\Gamma$ respectively and let $\phi:\Gamma'\rightarrow{\Gamma}$ be a surjective continuous map.

 The map $\phi$ is called a $(V(\Gamma'),V(\Gamma))$-morphism of (disconnected) $\Lambda$-metric graphs if the induced $\phi_{i,j}$ (as in Equation (\ref{MapsComponents1})) are $(V(\Gamma'_{i,j}),V(\Gamma_{i}))$-morphisms of $\Lambda$-metric graphs as in \cite[Definition 2.4]{ABBR1} with dilation factors $d_{e'}(\phi)\in\mathbb{Z}_{\geq{0}}$. 
The map $\phi$ is called a morphism of $\Lambda$-metric graphs if there exists a vertex set $V(\Gamma')$ of $\Gamma'$ and a vertex set $V(\Gamma)$ of $\Gamma$ such that $\phi$ is a $(V(\Gamma'),V(\Gamma))$-morphism of $\Lambda$-metric graphs. We say that $\phi$ is finite if $d_{e'}(\phi)\neq{0}$ for any edge $e'\in{E(\Gamma')}$. 

Let $\phi:\Gamma'\rightarrow\Gamma$ be a morphism of $\Lambda$-metric graphs. We say that $\phi$ is {\it{harmonic}} at $p'\in\Gamma'_{i,j}\subset{\Gamma'}$ if the induced morphism $\phi_{i,j}$ from Equation (\ref{MapsComponents1}) is harmonic at $p'$. The morphism $\phi$ is {\it{harmonic}} if it is harmonic at every $p'\in\Gamma'$. The degree of $\phi$ is defined to be the sum of the degrees of the $\phi_{i,j}$. 
\end{mydef}
%Using these definitions, we see that $\phi$ is finite if and only $\phi^{-1}(p)$ is a finite set for any point $p\in\Gamma$. In this paper we will only work with $\phi$ that are finite in this sense.

\begin{mydef}{\it{(Augmented metric graphs)}}\label{AugmentedMetricGraph}
An augmented $\Lambda$-metric graph is a $\Lambda$-metric graph $\Gamma$ as in Definition \ref{MetricGraphsVertexSets} with a function $g:\Gamma\rightarrow{\mathbb{Z}_{\geq{0}}}$ such that $g(p)=0$ for all points of $\Gamma$ except possibly for finitely many $\Lambda$-points $p\in\Gamma$. %The essential vertices of $\Gamma$ are the the points $p$ for which $\mathrm{val}(p)\neq{2}$ or $g(p)>0$. 
We now define a vertex set of $\Gamma$ to be a vertex set $V(\Gamma)$ as in Definition \ref{MetricGraphsVertexSets} of the underlying metric graph which contains all essential vertices of $\Gamma$. %as an augmented graph.  
A {\it{harmonic morphism}} of augmented $\Lambda$-metric graphs $\phi:\Gamma'\rightarrow{\Gamma}$ is then defined as a map which is a harmonic morphism between the underlying metric graphs of $\Gamma'$ and $\Gamma$, see Definition \ref{MorphismMetricGraph1}. 
\end{mydef}

%\begin{mydef}{\it{(\'{E}tale morphisms)}}
%Let $\phi:\Gamma'\rightarrow{\Gamma}$ be a finite harmonic morphism of augmented $\Lambda$-metric graphs as in Definition \ref{AugmentedMetricGraph}. We say that $\phi$ is \'{e}tale at a point $p'\in\Gamma'_{i,j}\subset{\Gamma'}$ if the restricted morphism $\phi_{i,j}$ is \'{e}tale at $p'$. We say that $\phi$ is (generically) \'{e}tale if the $\phi_{i,j}$ are (generically) \'{e}tale.
%\end{mydef}

\begin{mydef}{\it{(Disconnected metrized complexes)}}\label{MetrizedComplexDefinition}
A (disconnected) $\Lambda$-metrized complex of $k$-curves is an augmented $\Lambda$-metric graph $\Gamma$ (as in Definition \ref{AugmentedMetricGraph}) such that every connected component $\Gamma_{i}$ is a metrized complex as in \cite[Definition 2.17]{ABBR1}. 
\begin{comment}
\begin{itemize}
\item An augmented $\Lambda$-metric graph $\Gamma$ equipped with the choice of a distinguished vertex set $V(\Gamma)$.
\item For every finite vertex $p$ of $\Gamma$, a smooth, proper, connected $k$-curve $C_{p}$ of genus $g(p)$.
\item An injective function $\mathrm{red}_{p}:T_{p}(\Gamma)\rightarrow{C_{p}(k)}$, called the reduction map. The image of $\mathrm{red}_{p}$ is the set of {\it{marked points}} on $C_{p}$. 
\end{itemize}
\end{comment}
\end{mydef}


\begin{mydef}{\it{(Harmonic morphisms of metrized complexes)}}\label{HarmonicMorphism1}
A {\it{harmonic morphism of metrized complexes of curves}} as introduced in Definition \ref{MetrizedComplexDefinition} consists of the following data:
\begin{itemize}
\item A harmonic $(V(\Gamma'),V(\Gamma))$-morphism $\phi:\Gamma'\rightarrow{\Gamma}$ of augmented metric graphs as in Definition \ref{AugmentedMetricGraph},
\item For every finite vertex $p'$ of $\Gamma'$ with $d_{p'}>0$ a finite morphism of curves $\phi_{p'}:C'_{p'}\rightarrow{C_{\phi(p')}}$ such that the $(V(\Gamma'_{i,j}),V(\Gamma_{i}))$-morphisms $\phi_{i,j}$ of Equation (\ref{MapsComponents1}) induce morphisms of metrized complexes of $k$-curves as introduced in \cite[Definition 2.19]{ABBR1}. 
\end{itemize}

We say that a morphism $\phi:\Sigma'\rightarrow{\Sigma}$ of (disconnected) metrized complexes of curves is {\it{finite}}, {\it{tame}} or {\it{generically \'{e}tale}} % covering}}/{\it{tame harmonic morphism}}/{\it{tame covering}}/{\it{generically \'{e}tale covering}} 
if the morphisms on the connected components in Equation (\ref{MapsComponents1}) have the corresponding property as introduced in \cite[Section 2.16]{ABBR1}. We similarly define tame harmonic morphisms and tame coverings. 
\end{mydef}

\begin{exa}\label{ExampleFiberProduct}
We give an example of two tame coverings of metrized complexes such that the fiber product doesn't exist in the original category of connected coverings of a single metrized complex. The fiber product turns out to be the disjoint union of two metrized complexes. The example was set-up to be analogous to the fiber product of two copies of the morphism $\mathrm{Spec}(\mathbb{C})\rightarrow{\mathrm{Spec}(\mathbb{R})}$. 

Suppose that $\mathrm{char}(k)\neq{2}$. Let $\phi_{i}:C_{x'_{i}}\rightarrow{C_{x_{i}}}$ for $i=1,2$ denote the covering of projective lines given locally by $t\mapsto{t^{2}}$. We consider the finite tame covering of metrized complexes indicated in Figure \ref{Plaatje1}. That is, the curves $C_{x_{i}}$ and $C_{x'_{i}}$ correspond to the finite vertices and the leaves correspond to the branch/ramification points of the $\phi_{i}$. We also choose some identification of the inner edges with points on the curves $C_{x_{i}}$ and $C_{x'_{i}}$. The corresponding tame covering of metrized complexes will be denoted by $\Sigma'\rightarrow{\Sigma}$. Note that there is an action of $\mathbb{Z}/2\mathbb{Z}$ on $\Sigma'$ such that $\Sigma'/\mathbb{Z}/2\mathbb{Z}=\Sigma$. We will denote the nontrivial automorphism by $\sigma$. 

The fiber product of $\Sigma'\rightarrow{\Sigma}$ over itself is then in fact a disjoint union of two copies of $\Sigma'\rightarrow{\Sigma}$, albeit with different projection maps. These projection maps are given by $(\mathrm{id},\sigma)$ and $(\sigma,\mathrm{id})$.    %We will give the corresponding projection maps,  nontrivial automorphism of order two.
\begin{figure}[h!]
\centering
\includegraphics[width=10cm]{{Plaatje1-2.png}}
\caption{\label{Plaatje1} The fiber product in the category of coverings of metrized complexes in Example \ref{ExampleFiberProduct}. }%
\end{figure}

In Example \ref{EllipticCurveExample1}, we will see that these coverings naturally arise from the degree two covering on an elliptic curve with multiplicative reduction. 
  
\end{exa}
\begin{rem}
Throughout this paper, we will assume that our metrized complexes $\Sigma$ are {\it{loopless}}. That is, $\Sigma$ contains no edges whose closure is homeomorphic to a circle.  
\end{rem}

\subsection{Semistable vertex sets and triangulated punctured curves}

We now review the notion of semistable vertex sets and triangulated punctured curves, where we again expand upon the definition of \cite{ABBR1} by allowing disconnected algebraic curves.

Let $X$ be a smooth, proper algebraic $K$-curve and let $X_{i}$ be its irreducible (and connected) components. For every $X_{i}$, let $D_{i}\subseteq{X_{i}(K)}$ be a finite set of closed points. We naturally have $$X^{\mathrm{an}}=(\coprod{X_{i}})^{\mathrm{an}}=\coprod{(X_{i})^{\mathrm{an}}},$$ so we can analytify every irreducible component separately and consider all the notions in \cite{ABBR1} per connected component. We will write $D:=\coprod{D_{i}}$. 

\begin{mydef}\label{Semistablevertexset1}
A {\it{semistable vertex set}} of $(X,D)$ is a collection of semistable vertex sets $V_{i}$ for all the marked irreducible components $(X_{i},D_{i})$ of $X$. That is, it is a finite set of type-$2$ points for every $X_{i}^{\mathrm{an}}$ such that $X_{i}^{\mathrm{an}}\backslash{V_{i}}$ is a disjoint union of open balls and finitely many open annuli, where the points of $D_{i}$ are contained in distinct open ball connected components. We will write this collection of semistable vertex sets for $(X,D)=\coprod{(X_{i},D_{i})}$ as $V=\coprod{V_{i}}$.
\end{mydef}
\begin{mydef}{\it{(Triangulated punctured curves)}}
A {\it{triangulated punctured curve}} $(X,V\cup{D})$ is a smooth proper algebraic curve together with a finite set $D_{i}$ of {\it{punctures}} for every irreducible component $X_{i}$ of $X$ and a semistable vertex set $V$ for $(X,D)$ as in Definition \ref{Semistablevertexset1}.
\end{mydef}

\begin{mydef}{\it{(Skeleton of a triangulated punctured curve)}}
Let $(X,V\cup{D})$ be a triangulated punctured curve. The {\it{skeleton}} $\Sigma(X,V\cup{D})$ of $(X,V\cup{D})$ is the disjoint union of the skeleta of the connected triangulated punctured curves $(X_{i},V_{i}\cup{}D_{i})$, corresponding to the irreducible components $X_{i}$ of $X$.
\end{mydef}

\begin{mydef}\label{TriangulatedPuncturedCurveMorphism}
{\it{(Finite morphisms of triangulated punctured curves)}}
Let $(X,V\cup{D})$ and $(X',V'\cup{D'})$ be triangulated punctured curves. A finite morphism $(X',V'\cup{D'})\rightarrow{(X,V\cup{D})}$ of triangulated punctured curves is a finite morphism $\phi:X'\rightarrow{X}$ such that $\phi^{-1}(D)=D'$, $\phi^{-1}(V)=V'$ and $\phi^{-1}(\Sigma(X,V\cup{D}))=\Sigma(X',V'\cup{D'})$ as sets.
\end{mydef}


For any semistable vertex set $V$ of $(X,D)$, there is a natural retraction map $\tau_{V}:X^{\mathrm{an}}\rightarrow{\Sigma(X,V\cup{D})}$ by taking the retraction maps on the induced connected triangulated punctured curves $\tau_{V_{i}}:X_{i}^{\mathrm{an}}\rightarrow{\Sigma(X_{i},V_{i}\cup{D_{i}})}$. See \cite[Definition 3.7]{BPRa1} for the definition of retraction map in the connected case. If $V$ is clear from context, we will just denote this retraction by $\tau$. %We will denote this map by $\tau$ if the semistable vertex $V$ is clear from context.  
%We now define the retraction map for any semistable vertex set $V$ of $X^{\mathrm{an}}$. 

\begin{comment}


\subsection{Semistable models}\label{SemistableModels1}

In this section, we will review the correspondence between semistable models of an algebraic curve $X$ and semistable vertex sets thereof, as outlined in \cite[Section 5]{ABBR1}. %We will furthermore define the reduction map and give the {\it{"Slope formula"}}, which will be one of the main ingredients in the characterization of the abelianization of the fundamental group in Section \ref{Abelianization1}.

Let $X$ be a smooth, proper, connected algebraic curve over $K$. A (strongly) semistable model $\mathcal{X}$ of $X$ is a flat, integral, scheme $\mathcal{X}\rightarrow{\mathrm{Spec}(R)}$ whose special fiber $\mathcal{X}_{s}$ is a (strongly) semistable curve. That is, it is a reduced curve whose singularities are at worst ordinary double points. It is strongly semistable if additionally the irreducible components are nonsingular. Since $\mathcal{X}$ is proper over $R$, any $K$-point $x\in{X(K)}$ lifts uniquely to an $R$-point of $\mathcal{X}$. We define the reduction $\mathrm{red}(x)$ of $x$ to be the special fiber of this $R$-point. Writing $X^{0}$ for the closed points of $X$, we thus have a map
\begin{equation}
\mathrm{red}_{\mathcal{X}}:X^{0}\rightarrow{\mathcal{X}_{s}(k)}.
\end{equation}
Let $D\subset{X(K)}$ be a finite set. A semistable model $\mathcal{X}$ for $(X,D)$ is a semistable model for $X$ such that the points of $D$ reduce to distinct smooth points of $\mathcal{X}_{s}$ under $\mathrm{red}_{\mathcal{X}}$.

We now similarly define (strongly) semistable {\it{formal}} $R$-models of $X$. A (strongly) semistable formal $R$-model is an integral, proper, admissible formal $R$ curve $\mathfrak{X}$ whose analytic generic fiber $\mathfrak{X}_{K}$ is equipped with an isomorphism to the analytification $X^{\mathrm{an}}$ and whose special fiber $\mathfrak{X}_{s}$ is a (strongly) semistable curve. The $\varpi$-adic completion functor then defines an equivalence from the category of semistable $R$-models of $X$ to semistable formal $R$-models of $X$, see \cite[Lemma 5.1]{ABBR1}.  


For any integral admissible formal $R$-model, we again have a surjective reduction map
\begin{equation}
\mathrm{red}:X^{\mathrm{an}}\rightarrow{\mathfrak{X}_{s}},
\end{equation}
which is now anti-continuous, in the sense that the inverse image of a Zariski open set is closed in $X^{\mathrm{an}}$. We then have the following characterization of the inverse images of the points in $\mathfrak{X}_{s}$ under the reduction map:
\begin{theorem}\label{SpecializationBerkovich1}
Let $\mathfrak{X}$ be an integral admissible formal $R$-model of $X$ and let $\overline{x}\in\mathfrak{X}_{s}$ be a point. Then
\begin{enumerate}
\item $\overline{x}$ is a generic point if and only if $\mathrm{red}^{-1}(\overline{x})$ consists of a single type-$2$ point of $X^{\mathrm{an}}$.
\item $\overline{x}$ is a smooth closed point if and only if $\mathrm{red}^{-1}(\overline{x})$ is an open ball.
\item $\overline{x}$ is an ordinary double point if and only if $\mathrm{red}^{-1}(\overline{x})$ is an open annulus.
\end{enumerate}
\end{theorem}
\begin{proof}
See \cite[Theorem 4.6]{BPRa1} for the current formulation of the theorem. The proof of the first statement can be found in \cite[Proposition 2.4.4]{berkovich2012} and the other two in \cite[Propositions 2.2 and 2.3]{Bosch1985}. 
\end{proof}

As in \cite[Section 5.6]{ABBR1}, we can now associate to every semistable formal model $\mathfrak{X}$ of $X$ a semistable vertex set:
\begin{equation}
V(\mathfrak{X})=\{\mathrm{red}^{-1}(\zeta): \,\zeta\in\mathfrak{X}_{s} \text{ is a generic point }\}.
\end{equation}
The corresponding association $\mathfrak{X}\mapsto{V(\mathfrak{X})}$ is a bijection between the set of (strongly) semistable formal models of $(X,D)$ and the set of (strongly) semistable vertex sets of $(X,D)$, see \cite[Theorem 5.8]{ABBR1}. 
We can now also assign a metrized complex $\Sigma(X,V(\mathfrak{X})\cup{D})$ to $\mathfrak{X}$ as follows. We let $V$ be the irreducible components of $\mathfrak{X}_{s}$, considered as vertices of a graph. For every $x\in{V}$, we will write $C_{x}$ for the corresponding irreducible component in $\mathfrak{X}_{s}$. To every double point $\overline{x}\in\mathfrak{X}_{s}$, we assign an edge of length $l(x)$, where $l(x)=\mathrm{val}(\varpi)$ for any $\varpi\in{K^{*}}$ such that
\begin{equation}
\hat{\mathcal{O}}_{\mathfrak{X},x}=R[[s,t]]/(st-\varpi).
\end{equation}

\subsection{The Slope formula}\label{SlopeFormulaSection}

We now review the {\it{Slope formula}}, relating the slope of the logarithm of an analytic function to the order of its reduction at a vertex of a semistable vertex set $V$. This will be one of the main ingredients in the characterization of the abelianization of the fundamental group in Section \ref{Abelianization1}.

Let $X$ be a connected smooth proper curve over $K$ and let $x\in{\mathbf{H}(X^{\mathrm{an}}):=X^{\mathrm{an}}\backslash{X(K)}}$. We will be following \cite[Section 5.11]{BPRa1}. Consider the set of geodesic segments $\alpha:[0,a]\rightarrow{\mathbf{H}(X^{\mathrm{an}})}$ starting at $x$ (see \cite[Section 5.8]{BPRa1} for the definition of a geodesic segment). We say two geodesic segments are equivalent if they agree on a neighborhood of $0$. We then define the set of {\it{tangent directions}} $T_{x}$ at $x$ to be the set of nontrivial geodesic segments up to equivalence. The most important case for us is that of a type-$2$ point. Here, we have that $x$ corresponds to an smooth irreducible component $\overline{\mathcal{C}}$ of a formal semistable model $\mathcal{C}$ and the tangent directions at $x$ correspond to the $k$-rational points of $\overline{\mathcal{C}}$:
\begin{equation}\label{TangentDirectionsPoints}
T_{x}\simeq{}\overline{\mathcal{C}}(k).
\end{equation}

Suppose again that $x\in{X^{\mathrm{an}}}$ is a type-$2$ point and let $f$ be an analytic function in a neighborhood of $x$. Let $c\in{K^{*}}$ be such that $|f(x)|=c$. We set $\tilde{f}_{x}$ to be the residue of $f/c$ in $\tilde{\mathcal{H}}(x)$. This depends on our choice of $c$, but only up to a constant factor in $k^{*}$. This $\tilde{f}_{x}$ was also called the $\overline{\mathcal{C}}$-modified form in \cite{tropabelian}, where it played a crucial role in determining the splitting behavior of the edges of the Berkovich skeleton in a finite covering.

We now say that a function $F:X^{\mathrm{an}}\rightarrow{\mathbb{R}}$ is {\it{piecewise linear}} if the pullback to any geodesic segment is piecewise affine. For any piecewise linear function $F:X^{\mathrm{an}}\rightarrow{\mathbb{R}}$, we define the outgoing slope of $F$ at $x$ in the direction of $v\in{T_{x}}$ to be the slope of the pullback of $F$ to a geodesic segment representing $v$ in the direction of $v$, see \cite[Definition 5.14]{BPRa1}. We denote this slope by $d_{v}F(x)$. We then say $F$ is {\it{harmonic}} at $x$ if $d_{v}F(X)$ is nonzero for only finitely many $v$ and $\sum_{v\in{T_{x}}}d_{v}F(x)=0$. We say that $F$ is harmonic if it is harmonic at all $x\in\mathbf{H}(X^{\mathrm{an}})$. 




Let us now state the {\it{Slope formula}}. In short, it says that the logarithm of an analytic function $f$ is piecewise linear and we can express the slopes of this piecewise linear function in terms of quantities associated to $f$.  We will mostly be needing this association for type-$2$ points, where it equates the slope of the logarithm $F:=-\mathrm{log}|f|$ of an analytic function $f$ in a tangent direction $v$ at a point $x$ to the order of its reduction $\tilde{f}_{x}$ at the point $\tilde{v}\in\overline{\mathcal{C}}(k)$ corresponding to the tangent direction by Equation (\ref{TangentDirectionsPoints}).  %at a vertex of a semistable vertex set.  \todo{Toevoegen raakrichtingen}
\begin{theorem}{\it{(Slope formula)}}\label{SlopeFormula1}
Let $(X,D)$ be a punctured curve, let $V$ be a semistable vertex set for $(X,D)$ and let $\Sigma=\Sigma(X,V\cup{D})$ be its skeleton. Let $f$ be an algebraic function with no poles or zeros on $X\backslash{D}$ and let $F:=-\mathrm{log}(|f|):X^{\mathrm{an}}\rightarrow{\mathbb{R}}$. Then
\begin{enumerate}
\item $F=F\circ{\tau_{\Sigma}}$ on $X^{\mathrm{an}}\backslash{D}$, where $\tau_{\Sigma}:X^{\mathrm{an}}\rightarrow{\Sigma}$ is the retraction map. 
\item $F$ is piecewise-linear with integer slopes, and $F$ is affine linear on every edge of $\Sigma$. 
\item If $x$ is a type-$2$ point of $X^{\mathrm{an}}$ and $v\in{T_{x}}$ then $d_{v}(F(x))=\mathrm{ord}_{v}(\tilde{f}_{x})$. 
\item $F$ is harmonic.
\item Let $x\in{D}$, let $e$ be the infinite ray in $X^{\mathrm{an}}$ whose closure contains $x$, let $y\in{V}$ be the other endpoint of $e$ and let $v$ be the tangent direction corresponding to $e$. Then $d_{v}F(y)=\mathrm{ord}_{x}(f)$. 
\end{enumerate} 
\end{theorem}
\begin{proof}
See \cite[Theorem 5.15]{BPRa1}. 
\end{proof}

\end{comment}



\subsection{Lifting tame coverings of disconnected metrized complexes}

\label{TameCoverings1}\label{CoveringConnected1}\label{CoveringDisconnected1}


%\end{rem}
\begin{comment}
\subsubsection{Lifting connected tame coverings of metrized complexes}\label{CoveringConnected1}

 Let $X$ be a smooth, proper, connected curve over $K$ and let $x\in{X^{\mathrm{an}}}$ be a type-$2$ point. Let $V$ be a strongly semistable vertex set of $X$ containing $x$, let $\Sigma=\Sigma(X,V)$ and let $\tau:X^{\mathrm{an}}\rightarrow{\Sigma}$ be the retraction onto the skeleton. Let $e_{1},...,e_{r}$ in $\Sigma$ be the edges adjacent to $x$ and consider $\Sigma_{0}=\{x_{0}\}\cup{e_{1}^{o}}\cup{...}\cup{e_{r}^{o}}$. Here $e^{o}$ denotes the edge $e$ without its endpoints. Consider the open neighborhood $\tau^{-1}(\Sigma_{0})$ of $x$ in $X^{\mathrm{an}}$. These neighborhoods are known as {\it{simple}} or {\it{elementary}} neighborhoods of $x$, see \cite[Definition 4.28]{BPR11} and \cite[Section 3.6]{Berkovich1993}. We will refer to them as simple neighborhoods of $x$. 
\begin{mydef}
A {\it{star-shaped curve}} is a pointed $K$-analytic space $(Y,y)$ which is isomorphic to $(U,x)$, where $x$ is a type-$2$ point in the analytification of a smooth, proper, connected curve over $K$ and $U$ is a simple neighborhood of $x$. 
A {\it{punctured star-shaped curve}} is a star-shaped curve $(Y,y)$ together with a set of points $D\subset{Y(K)}$ such that the points of $D$ are contained in distinct open ball connected components of $Y\backslash\{y\}$. The skeleton of a punctured star-shaped curve is the set
\begin{equation}
\Sigma(Y,\{y\}\cup{D})=\{y\}\cup{D}\cup\bigcup_{i=1}^{r}\Sigma(A_{i})\cup\bigcup_{j=1}^{s}\Sigma(B_{j}),
\end{equation}
where the $A_{i}$ are the annuli corresponding to the open edges $e_{1}^{o},...,e_{r}^{0}$ of $Y$ and the $B_{j}$ are open balls punctured at the points of $D\subset{Y(K)}$. 

\end{mydef}

\begin{mydef}
A {\it{tame covering}} $(Y',y',D')\rightarrow{(Y,y,D)}$ of punctured star-shaped curves $(Y',y',D')$ and ${(Y,y,D)}$ is a finite morphism $\phi:Y'\rightarrow{Y}$ of $K$-analytic spaces satisfying the following properties:
\begin{enumerate}
\item $\phi^{-1}(y)=\{y'\}$,
\item $D'=\phi^{-1}(D)$, and 
\item if $C_{y'}$ denotes the residue curve of $Y'$ and $\phi_{y'}:C_{y'}\rightarrow{C_{y}}$ is the morphism induced by $\phi$, then $\phi_{y'}$ is tamely ramified and is branched only over the points of $C_{y}$ corresponding to tangent directions at $y$ represented by edges in $\Sigma_{0}=\Sigma(Y,\{y\}\cup{D})$.
\end{enumerate}
\end{mydef}

We now have the following theorem:
\begin{theorem}\label{UniqueLiftingStarShaped}{\it{(Local lifting theorem)}}
Let $(Y,y,D)$ be a punctured star-shaped curve with skeleton $\Sigma_{0}=\Sigma(Y,\{y\}\cup{D})$ and residue curve $C_{y}$, let $C'$ be a smooth, proper, connected $k$-curve, and let $\overline{\phi}:C'\rightarrow{C_{y}}$ be a finite, tamely ramified morphism branched only over the points of $C_{y}$ corresponding to tangent directions at $y$ represented by edges in $\Sigma_{0}$. Then there exists a lifting of $C'$ to a punctured star-shaped curve over $(Y,y,D)$, and this lifting is unique up to unique isomorphism.
\end{theorem}
\begin{proof}
See \cite[Theorem 6.18]{ABBR1}.
\end{proof}

In other words, we can uniquely lift the local algebraic structure over $k$ of a morphism of curves to a $K$-analytic structure. These local liftings are the main ingredients in passing from a covering of a metrized complex of $k$-curves $\Sigma$ to a covering of an algebraic curve $X$. To do this, one glues together these local liftings to obtain a proper analytic morphism $X'^{\mathrm{an}}\rightarrow{X^{\mathrm{an}}}$, which must come from an algebraic morphism $X'\rightarrow{X}$ by GAGA (which is \cite[Corollary 3.4.13]{berkovich2012} in the analytic case). We will first say what we mean by a lifting of a tame covering and then we will pinpoint this gluing data that allows us to find an appropriate algebraic covering.

Let us fix a triangulated punctured curve $(X,V\cup{D})$ with skeleton $\Sigma=\Sigma(X,V\cup{D})$ let $\tau:X^{\mathrm{an}}\rightarrow{\Sigma}$ be the canonical retraction. Assume that $\Sigma$ has no loop edges and let $\phi:\Sigma'\rightarrow{\Sigma}$ be a tame covering of connected metrized complexes of $k$-curves.
\begin{mydef}
A {\it{lifting}} of $\Sigma'\rightarrow{\Sigma}$ to a tame covering of $(X,V\cup{D})$ is a tame covering of triangulated punctured curves $\phi:(X',V'\cup{D'})\rightarrow{(X,V\cup{D})}$ equipped with a $\Sigma$-isomorphism $\phi^{-1}(\Sigma)\simeq{\Sigma'}$ of connected metrized complexes of $k$-curves.
\end{mydef}

Our goal is to first construct a lifting of $\Sigma'\rightarrow{\Sigma}$. Let $x\in{V}$ be a finite vertex. There is a canonical punctured star-shaped associated to $x$: we take the connected component $\Sigma(x)$ of $x$ in $\{x\}\cup(\Sigma\backslash{V})$ and let $Y(x):=\tau^{-1}(\Sigma(x))$ be the corresponding simple neighborhood. Let $D(x)=D\cap{Y(x)}$. Then $(Y(x),x,D(x))$ is a punctured star-shaped curve. The morphism $\phi_{x}:C_{x'}\rightarrow{C_{x}}$ from the data of a morphism of metrized complexes is finite, tamely ramified and branched only over the points of $C_{x}$ corresponding to tangent directions at $x$ represented by edges of $\Sigma(x)$. By Theorem \ref{UniqueLiftingStarShaped}, there is a unique lifting of $C_{x'}\rightarrow{C_{x}}$ to a covering of punctured star-shaped curves. We denote that lifting by $Y(x')\rightarrow{Y(x)}$. We let $\tau_{x'}$ be the canonical retraction of $Y(x')$ onto its skeleton.

Let $e'\in{E_{f}(\Sigma')}$ and $e=\phi(e')$. Let $x',y'$ be the endpoints of $e'$. Choose $a,a'\in{K^{*}}$ such that $\mathrm{val}(a)=\ell(e)$ and $\mathrm{val}(a')=\ell(e')$. By \cite[Proposition 6.15(3)]{ABBR1}, there are isomorphisms
$\tau^{-1}(e^{o}) \simeq{\mathbf{S}(a)_{+}}$, 
$\tau^{-1}_{x}(e^{0})  \simeq{\mathbf{S}(a')_{+}}$
and 
$\tau^{-1}_{y}(e^{0})  \simeq{\mathbf{S}(a')_{+}}$
such that the corresponding morphisms to $\tau^{-1}(e^{o})$ are given by $t\mapsto{t^{d_{e'}(\phi)}}$, where $d_{e'}(\phi)$ is the degree of the edge map.  Let $E^{\pm}_{f}(\Sigma')$ denote the set of oriented finite edges of $\Sigma'$ and for $e'\in{E^{\pm}_{f}(\Sigma')}$, let $\overline{e}'$ denote the same edge with the opposite orientation. 
\begin{mydef}\label{GluingDataFirst}
{\it{(Gluing data)}}
The set of gluing data $\mathcal{G}(\Sigma',X)$ for a lifting of $\Sigma'$ to a tame covering of $(X,V\cup{D})$ is the set of tuples $(\Theta_{e'})_{e'\in{E^{\pm}_{f}(\Sigma')}}$ of isomorphisms
\begin{equation}
\tau^{-1}_{x'}(e'^{o})\simeq{\tau^{-1}_{y'}(e'^{o})}
\end{equation}
such that $\Theta_{\overline{e}'}=\Theta^{-1}_{e'}$.
\end{mydef}

We now recall the conjugation action of $\mathrm{Aut}_{\Sigma}(\Sigma')$ on the set of gluing data $\mathcal{G}(\Sigma',X)$. Let $x'\in{V_{f}(\Sigma')}$, $x''=\alpha(x')$ and $x=\phi(x')=\phi(x'')$. Every $\alpha\in\mathrm{Aut}_{\Sigma}(\Sigma')$ induces a $Y(x)$ isomorphism of star-shaped curves
\begin{equation}
Y'(x')\rightarrow{Y''(x'')},
\end{equation} which induces an isomorphism of annuli
\begin{equation}
\alpha_{x'}:\rightarrow{\tau^{-1}_{x'}(e'^{o})}\rightarrow{\tau^{-1}_{x''}(e''^{o})}.
\end{equation}

The conjugation action of $\mathrm{Aut}_{\Sigma}(\Sigma')$ on $\mathcal{G}(\Sigma',X)$ is defined by the rule
\begin{equation}
\alpha\cdot{(\Theta_{e'})}=(\alpha^{-1}_{y'}\circ{\Theta_{\alpha(e')}}\circ{\alpha_{x'}})%_{e'\in{E^{\pm}_{f}(\Sigma')}},
\end{equation}
where $e'=\overrightarrow{x'y'}$. 

We can now state the following {\it{classification theorem}} for lifts of tame coverings:
\begin{theorem}{\it{(Classification theorem for lifts of tame coverings)}}\label{ClassTheorem1}
Let $(X,V\cup{D})$ be a triangulated punctured curve with skeleton $\Sigma=\Sigma(X,V\cup{D})$. Assume that $\Sigma$ has no loop edges. Let $\phi:\Sigma'\rightarrow{\Sigma}$ be a tame covering of metrized complexes curves. Then
\begin{enumerate}
\item There is a canonical bijection between the set of gluing data $\mathcal{G}(\Sigma',X)$ and the set of liftings of $\Sigma'$ to a tame covering of $(X, V\cup{D})$, up to $X$-isomorphism preserving $\Sigma'$. In particular, there exists a lifting of $\Sigma'$. Any such lifting has no nontrivial automorphisms which preserve $\Sigma'$.
\item Two tuples of gluing data determine $X$-isomorphic curves if and only if they are in the same orbit under the conjugation action. The stabilizer in $\mathrm{Aut}_{\Sigma}(\Sigma')$ of an element of $\mathcal{G}(\Sigma',X)$ is canonically isomorphic to the $X$-automorphism group of the associated curve. 
\end{enumerate}
\end{theorem}
\begin{proof}
See \cite[Theorem 7.4]{ABBR1}.
\end{proof}

\end{comment}

%\subsubsection{Lifting disconnected tame coverings of metrized complexes}

%We now study  (possibly disconnected) liftings of tame coverings of metrized complexes. 
Let $\phi:\Sigma'\rightarrow{\Sigma}$ be a tame covering of metrized complexes as in Definition \ref{HarmonicMorphism1}, where we note that both $\Sigma'$ and $\Sigma$ can be disconnected. Let $\Sigma'_{i,j}$ be the connected components of $\Sigma'$ that map to the connected components $\Sigma_{i}$. By definition, there are induced morphisms of connected metrized complexes 
\begin{equation}
\phi_{i,j}:\Sigma'_{i,j}\rightarrow{\Sigma_{i}}.
\end{equation}

For every $i$, let $(X_{i},V_{i}\cup{D_{i}})$ be a triangulated punctured curve with skeleton $\Sigma_{i}$ and let $\tau_{i}:X^{\mathrm{an}}_{i}\rightarrow\Sigma_{i}$ be the canonical retraction. We assume again that every $\Sigma_{i}$ has no loop edges. 
\begin{mydef}\label{Lifting2}
A {\it{lifting}} of $\Sigma'\rightarrow{\Sigma}$ to a tame covering of $(X,V\cup{D})$ %$\coprod{(X_{i},V_{i}\cup{D_{i}})}$ 
is a set of liftings of $\Sigma'_{i,j}\rightarrow{\Sigma_{i}}$ to triangulated punctured curves $(X'_{i,j},V'_{i,j}\cup{D'_{i,j}})\rightarrow{(X_{i},V_{i}\cup{D_{i}})}$. Here liftings of connected curves are as defined in \cite[Section 7]{ABBR1}.
\end{mydef}

We can now define the set of gluing data for a general covering of metrized complexes. For the original definition of the gluing data for connected coverings, we refer the reader to \cite[Section 7.2]{ABBR1}.

\begin{mydef}\label{GluingData2}
Let $\mathcal{G}(\Sigma'_{i,j},X_{i})$ be the set of gluing data for a lifting of $\Sigma'_{i,j}\rightarrow{\Sigma_{i}}$ to a covering of $X_{i}$. We define the set of gluing data for a lifting of $\Sigma'\rightarrow{\Sigma}$ to be the product
\begin{equation}
\mathcal{G}(\Sigma',X):=\prod_{i}\mathcal{G}(\Sigma'_{i,j},X_{i}).
\end{equation}
\end{mydef}

As in \cite{ABBR1}, we now define the conjugation action of $\alpha$ on $\mathcal{G}(\Sigma',X)$. Let $\Sigma'_{i,j}$ be a connected component of $\Sigma'$ mapping to $\Sigma_{i}\subset{\Sigma}$. Let $\alpha\in\mathrm{Aut}_{\Sigma}(\Sigma')$, which is defined as the group of degree $1$ harmonic morphisms of $\Sigma'$ (as a metrized complex) that fix $\Sigma$. Since $\alpha$ fixes $\Sigma$ and thus $\Sigma_{i}$, we see that $\alpha$ maps $\Sigma'_{i,j}$ to another component above $\Sigma_{i}$. We will denote this component by $\Sigma'_{i,\alpha({j})}$. Let $x'\in{V_{f}(\Sigma'_{i,j})}$ and let $x''=\alpha(x')\in{V_{f}(\Sigma'_{i,\alpha(j)})}$ and $x=\phi(x')=\phi(x'')$. From \cite[Theorem 6.18]{ABBR1}, we obtain a unique lift of the corresponding morphism of residue curves $C_{x'}\rightarrow{C_{\alpha(x')}}$ to a $Y(x)$-isomorphism of star-shaped curves $Y'(x')\rightarrow{Y'(x'')}$.  Here a star-shaped curve is as defined in \cite[Definition 6.2]{ABBR1}. Let $e'\in{E_{f}(\Sigma'_{i,j})}$ be an edge adjacent to $x'$, $e''=\alpha(e')$ and let $e=\phi(e')=\phi(e'')$. From the isomorphism of star-shaped curves, we obtain an isomorphism 
\begin{equation}
\alpha_{x'}:\tau^{-1}_{x'}(e'^{o})\rightarrow{\tau^{-1}_{x''}(e''^{o})}.
\end{equation}

We define the conjugation action of $\mathrm{Aut}_{\Sigma}(\Sigma)$ by the rule
\begin{equation}\label{ConjugationAction}
\alpha\cdot{(\Theta_{e'})}=(\alpha^{-1}_{y'}\circ{\Theta_{\alpha(e')}}\circ{\alpha_{x'}})%_{e'\in{E^{\pm}_{f}(\Sigma'_{i,\alpha(j)})},
\end{equation}
where $e'=\overrightarrow{x'y'}$. We now easily deduce the following theorem, which is the disconnected version of \cite[Theorem 7.4]{ABBR1}. %Similar to \cite[Theorem 7.4]{ABBR1}, we now have 

\begin{theorem}\label{ClassTheorem2}
Let $(X,V\cup{D})$ be a triangulated punctured curve with skeleton $\Sigma$ and let $\Sigma'\rightarrow{\Sigma}$ %:=\coprod{\Sigma_{i}}}$ 
be a tame covering of (possibly disconnected) metrized complexes of curves.  Then
\begin{enumerate}
\item There is a bijection between the set of liftings of $\Sigma'$ to a tame covering of $X$ as in Definition \ref{Lifting2} (up to $X$-isomorphism preserving $\Sigma'$), and the set of gluing data $\mathcal{G}(\Sigma',X)$ as in Definition \ref{GluingData2}. %In particular, there exists a lifting of $\Sigma'$. 
Any such lifting has no nontrivial automorphisms which preserve $\Sigma'$.
\item Two tuples of gluing data $\Theta_{1}$ and $\Theta_{2}$ determine $X$-isomorphic curves if and only if there exists an $\alpha\in{\mathrm{Aut}_{\Sigma}(\Sigma')}$ such that $\alpha\cdot{}(\Theta_{1})=\Theta_{2}$. Here the conjugation action is as defined in Equation (\ref{ConjugationAction}). % are in the same orbit under the conjugation action defined in Equation \ref{ConjugationAction}: $\alpha\cdot{}\Theta_{1}=\Theta_{2}$.
The stabilizer $\mathrm{Stab}(\Theta)$ in $\mathrm{Aut}_{\Sigma}(\Sigma')$ of an element $\Theta$ of $\mathcal{G}(\Sigma',X)$ is canonically isomorphic to the $X$-automorphism group of the associated curve. 
\end{enumerate}
\end{theorem}
\begin{proof}
%Using Definitions \ref{Lifting2} and \ref{GluingData2}, 
This follows as in \cite[Theorem 7.4]{ABBR1}. We leave the details to the reader. 

\end{proof}

\begin{comment}

\begin{exa}
Let $X$ be a curve of genus $2$ with skeleton $\Sigma$ as in Figure [...]. For instance, the curve defined by the equation 
\begin{equation}
y^2=x(x-\varpi)(x+1)(x+1-\varpi)(x+2)(x+2-\varpi)
\end{equation}
has $\Sigma$ as its skeleton. Note that $\Sigma$ has no leaves.
%whose skeleton 
For any tame covering $\phi_{\Sigma}:\Sigma'\rightarrow{\Sigma}$, we obtain from Theorem \ref{ClassTheorem2} a covering $X'\rightarrow{X}$ of algebraic curves such that the induced covering on graphs is $\phi_{\Sigma}$. Let $\pi(\Sigma)$ be the topological fundamental group. This is isomorphic to the free group on two letters $a$ and $b$. For any tame subgroup of finite index, we obtain a covering of $\Sigma$ and thus a covering of $X$. The normal subgroup $H:=(a^4,b^2,baba)$ has index $8$ and the quotient $\pi(\Sigma)/H$ is isomorphic to the dihedral group $D_{8}$, which is the symmetry group of a square. For $\mathrm{char}(k)\neq{2}$, this covering of metrized complexes is tame. By Theorem \ref{ClassTheorem2}, there is an algebraic covering $X'\rightarrow{X}$ which induces $\phi_{\Sigma}$. Furthermore, the action extends to $X'$ and we have $X'/D_{8}=X$. By the Riemann-Hurwitz formula, we then easily obtain that $g(X')=9$. %It will follow from the general theory that there is an action of $D_{8}$ on $X'$ such that $X'/D_{8}=X$. 

\end{exa}

\end{comment}


\subsection{Tropical Jacobians}\label{TropicalJacobians}

We now define the {\it{Tropical Jacobian}} of a finite metric graph, which will be used in Section \ref{Abelianization1}. There are multiple possible references for this material, to name a few: \cite{Baker2014}, \cite{Bolognese2017} and \cite[Page 203]{MZ1}. We will mostly be following \cite[Section 3]{Baker2014}.

Let $X$ be a smooth proper connected $K$-curve and let $\Gamma$ be the intersection graph of a semistable formal $R$-model, considered as a metric graph. This graph can also be turned into a metrized complex, but we will only need the metric graph structure in this section. %As we saw in Section \ref{SemistableModels1}, we can even turn this intersection graph into a metrized complex, but we will only consider its associated metric graph structure in this subsection. 
We let $\Gamma(\Lambda)$ denote the set of all points of $\Gamma$ whose distance from any vertex belongs to $\Lambda$. Consider the canonical surjective retraction map
\begin{equation}
\tau:X^{\mathrm{an}}\rightarrow{\Gamma}.
\end{equation}
We then also obtain a map $\tau_{*}:\mathrm{Div}(X)\rightarrow{\mathrm{Div}_{\Lambda}(\Gamma)}$ by extending $\tau$ linearly, which induces a induced map on the divisors of degree zero $\tau_{*}:\mathrm{Div}^{0}(X)\rightarrow{\mathrm{Div}^{0}_{\Lambda}(\Gamma)}$. 
 We now define the notion of principal divisors on $\Gamma$. A {\it{tropical meromorphic function}} on $\Gamma$ is a continuous function $F:\Gamma\rightarrow{\mathbb{R}}$ which is piecewise affine with integer slopes. It is $\Lambda$-rational provided that $F(\Gamma(\Lambda))\subset{\Lambda}$ and all points at which $F$ is not differentiable are contained in $\Gamma(\Lambda)$.  We then define the divisor of $F$ to be
\begin{equation}
\mathrm{div}(F)=\sum_{x\in{\Gamma(\Lambda)}}n_{x}(x),
\end{equation}
where $n_{x}$ is the sum of the outgoing slopes of $F$ at $x$. The group of ($\Lambda$-rational) principal divisors on $\Gamma$ is then the subgroup $\mathrm{Prin}_{\Lambda}(\Gamma)\subset{\mathrm{Div}^{0}_{\Lambda}(\Gamma)}$ of divisors of $\Lambda$-rational tropical meromorphic functions. 

For any rational function $f\in{K(X)}$, we let $F$ be the restriction of $-\mathrm{log}(|f|)$ to $\Gamma$. By the Poincar\'{e}-Lelong formula (See \cite[Section 5]{BPRa1} and \cite[Proposition 3.3.15]{thuil1}), we see that $F$ is a $\Lambda$-rational tropical meromorphic function on $\Gamma$ and that $\tau_{*}(\mathrm{div}(f))=\mathrm{div}(F)$. In the algebraic case of a strongly semistable regular model, this theorem follows from intersection theory, see \cite[Section 3]{tropabelian}.  At any rate, we can now define the following:

\begin{mydef}\label{TropicalJacobian1}
Let $\Lambda=\mathbb{R}$. We define the {\it{Tropical Jacobian}} of $\Gamma$ to be the group
\begin{equation}
\mathrm{Jac}(\Gamma):=\mathrm{Div}^{0}_{\Lambda}(\Gamma)/\mathrm{Prin}_{\Lambda}(\Gamma).
\end{equation}
\end{mydef}

One can alternatively define the Tropical Jacobian using differential forms as follows. Let $H_{1}(\Gamma,\mathbb{Z})$ be the first singular homology group of $\Gamma$. Using the integration pairing $\gamma\mapsto{\int_{\gamma}}$, we obtain a map
\begin{equation}
\mu:H_{1}(\Gamma,\mathbb{Z})\rightarrow{\mathrm{Hom}(\Omega_{\Gamma(\Lambda)}(\Gamma),\Lambda)}
\end{equation}
By \cite[Proposition 3.8]{Baker2014}, we then have an isomorphism
\begin{equation}
\mathrm{Jac}(\Gamma)\simeq{{\mathrm{Hom}(\Omega_{\Gamma(\mathbb{R})}(\Gamma),\mathbb{R})/\mu(H_{1}(\Gamma,\mathbb{Z}))}}.
\end{equation}
In particular, we obtain an isomorphism of the Tropical Jacobian with the real torus $\mathbb{R}^{g}/\mathbb{Z}^{g}$, where $g=\mathrm{rank}_{\mathbb{Z}}(H_{1}(G,\mathbb{Z}))=\beta(\Gamma)$, the first Betti number of $\Gamma$. 





==> GaloisCategories.tex <==
\subsection{Galois categories}\label{GaloisCategories}

\todo{Verwijderen?}

In this section we review the notion of Galois categories. We will use the definition found in \cite[\href{https://stacks.math.columbia.edu/tag/0BMQ}{Tag 0BMQ}]{stacks-project} and we refer the reader to \cite{SGA1},  \cite{Lenstra} and \cite{Cadoret2013} for more background on the subject. In this paper we will be mainly interested in the category of residually tame coverings of an punctured algebraic curve $X\backslash{D}$, which forms a Galois category with profinite fundamental group $\pi_{\mathrm{Tame}}(X,D)$. % We will show in this section that this indeed forms a Galois category. 
In Section \ref{RigidifiedCoverings}, we will show that the category of enhanced tame coverings of a metrized complex is equivalent to this category, giving a definition of a tropical fundamental group. We will study this tropical fundamental group in Section \ref{TropicalFundamental}.  %isomorphism of the corresponding profinite fundamental groups. This equivalence will be given in Section \ref{AlgebraicMetrizedCoverings}.

Let $\mathcal{C}$ be a category. We assume here that $\mathcal{C}$ is essentially small.  %category. %Let $\mathcal{C}$ be an essentially small category. 
%Let $\mathcal{C}$ be such a category. 
For any $\phi\in\mathrm{Ar}(\mathcal{C})$, we say that $\phi$ is a {\it{monomorphism}} if it is left cancellative. That is, $f:X\rightarrow{Y}$ is a monomorphism if for any two morphisms $g_{i}:Z_{i}\rightarrow{X}$ in $\mathcal{C}$ such that $f\circ{g_{1}}=f\circ{g_{2}}$, we have $g_{1}=g_{2}$. A {\it{connected}} object of $\mathcal{C}$ is a non-initial object $X$ such that any monomorphism $Y\rightarrow{X}$ is initial or an isomorphism. Let $F$ be a functor $\mathcal{C}\rightarrow{\mathcal{D}}$. We say that $F$ is {\it{exact}} if it commutes with finite limits and finite colimits. We say that $F$ {\it{reflects isomorphisms}} if for any $f\in\mathrm{Ar}(\mathcal{C})$, if $Ff$ is an isomorphism, then $f$ is an isomorphism.

\begin{mydef}\label{GaloisCategoryDefinition}
Let $\mathcal{C}$ be a category and let $F:\mathcal{C}\rightarrow{(\mathrm{Sets})}$ be a functor. The pair $(\mathcal{C},F)$ is a {\it{Galois category}} if
\begin{enumerate}
\item $\mathcal{C}$ has finite limits and colimits,
\item every object of $\mathcal{C}$ is a finite (possibly empty) coproduct of connected objects,
\item $F(X)$ is finite for every object $X\in\mathrm{Ob}(\mathcal{C})$ and
\item $F$ reflects isomorphisms and is exact.
\end{enumerate}
\end{mydef}

We refer to $F$ as the {\it{fundamental functor}} of the Galois category. We will sometimes also refer to $\mathcal{C}$ as the Galois category. The definition of a Galois category is completely categorical, so this structure is preserved under categorical equivalences. We can therefore define the notion of an {\it{induced Galois category structure}}. 

\begin{mydef}\label{InducedStructure}{\it{(Induced Galois category structure)}}
Let $(\mathcal{C},F)$ be a Galois category and suppose that there is an equivalence of categories $G:\mathcal{D}\rightarrow{\mathcal{C}}$. Let $F'$ be the induced functor $FG:\mathcal{D}\rightarrow{(\mathrm{Sets})}$ defined by $FG(X)=F(G(X))$. Then $(\mathcal{D},F')$ is the {\it{induced Galois category structure}} on $\mathcal{D}$.
\end{mydef}



%\begin{exa}
%We will follow \cite[Section 3.7]{Lenstra} and \cite[Example 2.7]{Cadoret2013}. Let $X$ be a topological space and consider the category $\mathrm{Cov}(X)$ of finite {\it{coverings}} of $X$. Here a finite covering $\phi:X'\rightarrow{X}$ is a finite %{(\footnote{That is, for every $x\in{X}$ we have that $\phi^{-1}(x)$ is finite.})} 
%continuous surjective map such that for every $x\in{X}$, there exists a neighborhood $U$ of $x$ such that $\phi^{-1}(U)$ is homeomorphic to a disjoint union of $n$ copies of $U$ for some $n\in\mathbb{N}$. The fundamental functor, denoted by $F_{x}$ for any point $x$ in $X$ is then given as follows: %To construct the appropriate Galois category, one constructs the following fundamental functor $F_{x}$: 
%one assigns to every covering $\phi:X'\rightarrow{X}$ the inverse image $\phi^{-1}(x)$ of $x$ under $\phi$. %((A Galois object in the resulting category is then a topological space $X'$ with a continuous group action of a finite group $G$ on it such that $X'/G=X$. We note that the corresponding profinite group $\pi(X,x)$ is the profinite completion of the ordinary fundamental group (\todo{Controleren, referentie}). ))
%\end{exa}


\begin{lemma}\label{GaloisObject}
Let $(\mathcal{C},F)$ be a Galois category. Then for any connected $X\in\mathrm{Ob}(\mathcal{C})$, we have
\begin{equation}
|\mathrm{Aut}(X)|\leq{|F(X)|}.
\end{equation}
\end{lemma}
\begin{proof}
See \cite[\href{http://stacks.math.columbia.edu/tag/0BN0}{Lemma 0BN0}]{stacks-project}. 
\end{proof}

\begin{mydef}
Let $(\mathcal{C},F)$ be a Galois category. We say that a connected object $X$ is a {\it{Galois object}} if 
\begin{equation}
|\mathrm{Aut}(X)|={|F(X)|}.
\end{equation}
\end{mydef}

For any Galois object $X$, we let $X/\mathrm{Aut}(X)$ be the coequalizer of the arrows $\sigma:X\rightarrow{X}$, where $\sigma\in\mathrm{Aut}(X)$. This exists by condition $(1)$ in the definition of a Galois category. We then have the following Lemma:
\begin{lemma}
Let $X$ be a Galois object. Then the coequalizer $X/\mathrm{Aut}(X)$ is the terminal object of $\mathcal{C}$. 
\end{lemma}
\begin{proof}
We first prove that the action of $\mathrm{Aut}(X)$ is transitive on $F(X)$. Suppose that there exist an $x$ and $y$ in $F(X)$ such that no $\sigma\in\mathrm{Aut}(X)$ maps $x$ to $y$. By the pigeonhole principle, there exist $\sigma_{1}$ and $\sigma_{2}$ with $\sigma_{1}\neq{\sigma_{2}}$ such that $\sigma_{1}(x)=\sigma_{2}(x)$. By \cite[\href{http://stacks.math.columbia.edu/tag/0BN0}{Lemma 0BN0,(7)}]{stacks-project} we conclude that $\sigma_{1}=\sigma_{2}$, a contradiction. The action is thus transitive. If we now use the fact that $F$ commutes with finite colimits together with the transitivity, then we easily see that %By using the fact that $F$ commutes with finite colimits and the fact that the action of $\mathrm{Aut}(X)$ is transitive on $F(X)$ (by , we easily see that 
$F(X/\mathrm{Aut}(X))$ is the singleton set, implying that $X/\mathrm{Aut}(X)$ is the terminal object of $\mathcal{C}$ by \cite[\href{http://stacks.math.columbia.edu/tag/0BN0}{Lemma 0BN0, (5)}]{stacks-project}. 
\end{proof}

%\begin{exa}
%For a topological space $X$, a Galois object in $\mathrm{Cov}(X)$ is a topological space $X'$ with a continuous group action of a finite group $G$ on it such that $X'/G=X$. For a connected normal scheme $X$ with function field $K(X)$, every Galois object is obtained as follows. We take a finite Galois extension $L$ of $K(X)$ with Galois group $G$ and consider the normalization $X'$ of $X$ in $L$. There is then a natural action of $G$ on $X'$ and we have $X'/G=X$.  
%\end{exa}

Let $F:\mathcal{C}\rightarrow{(\mathrm{Sets})}$ be a fundamental functor. %  $F:\mathcal{C}\rightarrow{(\mathrm{Sets})}$. 
An automorphism of $F$ is an invertible morphism of functors $F\rightarrow{F}$.
We then have a canonical injective map
\begin{equation}\label{ProfiniteGroup}
\mathrm{Aut}(F)\rightarrow{\prod_{X\in\mathrm{Ob}(X)}\mathrm{Aut}(F(X))}.
\end{equation}

Assigning the discrete topology to every set on the righthand side of Equation (\ref{ProfiniteGroup}) and the product topology to the product, we see that $\mathrm{Aut}(F)$ naturally has the structure of a {\it{profinite}} group if $F$. % is the fundamental functor of a Galois category.  
In particular, we see that $\mathrm{Aut}(F)$ is a topological group. We then also have natural continuous maps
\begin{equation}
\mathrm{Aut}(F)\times{F(X)}\rightarrow{F(X)}
\end{equation}
for every $X\in\mathrm{Ob}(\mathcal{C})$. Letting $G:=\mathrm{Aut}(F)$, we obtain an induced functor % that the functor $F$ induces a functor
\begin{equation}
\tilde{F}:\mathcal{C}\rightarrow{(\mathrm{Finite}\mhyphen G \mhyphen \mathrm{Sets})},
\end{equation}
where $(\mathrm{Finite}\hyp G \hyp \mathrm{Sets})$ is the category of finite sets with a continuous $G$-action. We will often denote this functor by $F$ again. 
We can now state the main theorem on Galois categories:
\begin{theorem}\label{MainTheoremGaloisCategories}
Let $(\mathcal{C},F)$ be a Galois category and let $\tilde{F}:\mathcal{C}\rightarrow{(\mathrm{Finite}\mhyphen G \mhyphen \mathrm{Sets})}$ be the induced functor. We then have 
\begin{enumerate}
\item $\tilde{F}$ is an equivalence of categories.  
\item If $\pi$ is any profinite group such that the categories $\mathcal{C}$ and $(\pi\hyp\mathrm{Sets})$ are equivalent by an equivalence that, composed with the forgetful functor $(\pi\hyp\mathrm{Sets})\rightarrow{(\mathrm{Sets})}$ yields the functor $F$, then $\pi$ and $\mathrm{Aut}(F)$ are canonically isomorphic. 
\item If $F$ and $F'$ are two fundamental functors for $\mathcal{C}$, then they are isomorphic.
\item If $\pi$ is a profinite group such that $\mathcal{C}$ and $(\pi\hyp\mathrm{Sets})$ are equivalent, then there is an isomorphism of profinite groups $\mathrm{Aut}(F)\simeq{\pi}$ that is canonically determined up to an inner automorphism of $\mathrm{Aut}(F)$.  
\end{enumerate}
\end{theorem}
\begin{proof}
See \cite[\href{http://stacks.math.columbia.edu/tag/0BN4}{Proposition 0BN4}]{stacks-project}.  
\end{proof}

\begin{rem}\label{EquivalentDefinition}{\it{(An equivalent definition)}}
%Let $\mathcal{C}$ be a category and let ${F}$ be a functor to $(\mathrm{Sets})$. 
The definition given in \cite{Lenstra}, \cite{Cadoret2013} and \cite{SGA1} for a Galois category seems different from the one given here, but it is in fact equivalent. % a definition for a Galois category is given, but it turns out to be equivalent to the one given here. %There, ${F}$ and $\mathcal{C}$ have to satisfy the following set of axioms:
%\begin{enumerate}
%\item $\mathcal{C}$ has a final object and and finite fiber products exist in $\mathcal{C}$. 
%\item Finite coproducts exist in $\mathcal{C}$ and categorical quotients by finite groups of automorphisms exist in $\mathcal{C}$.
%\item Any morphism $u:Y\rightarrow{X}$ in $\mathcal{C}$ factors as $u"\circ{u'}:Y\rightarrow{X'}\rightarrow{X''}$, where $u'$ is a strict epimorphism and $u''$ is a monomorphism which is an isomorphism onto a direct summand of $X$. 
%\item ${F}$ sends final objects to final objects and commutes with fiber products. 
%\item ${F}$ commutes with finite coproducts and quotients by finite groups and sends strict epimorphisms to strict epimorphisms.
%\item ${F}$ reflects isomorphisms. 
%\end{enumerate}
%These definitions are in fact equivalent. 
To see this, let $\mathcal{C}$ be any category that is equivalent to $(\mathrm{Finite}\mhyphen{G}\mhyphen{\mathrm{Sets}})$ for some profinite group $G$. Since $(\mathrm{Finite}\mhyphen{G}\mhyphen{\mathrm{Sets}})$ is a Galois category in both definitions with respect to the forgetful functor $(\mathrm{Finite}\mhyphen{G}\mhyphen{\mathrm{Sets}})\rightarrow{(\mathrm{Finite}\mhyphen{\mathrm{Sets}})}$, we see that $\mathcal{C}$ is a Galois category (using the induced Galois category structure).    %which is the category of finite sets with a continuous action by a profinite group $G$. 
%Then $\mathcal{C}$ automatically satisfies the conditions in both definitions with respect to the composed functor $\mathcal{C}\rightarrow{}(\mathrm{Finite}\mhyphen{G}\mhyphen{\mathrm{Sets}})\rightarrow{(\mathrm{Sets})}$. %Using either definition, we obtain an equivalence with  
By Theorem \ref{MainTheoremGaloisCategories} and \cite[Theorem 2.8]{Cadoret2013} (or \cite[Theorem 3.5]{Lenstra}), we obtain an equivalence with $(\mathrm{Finite}\mhyphen{G}\mhyphen{\mathrm{Sets}})$ using either definition, so we see that the two definitions are equivalent. 

%As noted in \cite[Section 2.1.1]{Cadoret2013}, these definitions are in fact equivalent. 
\end{rem}

\begin{exa}\label{ExampleLenstra1}
We will follow \cite[Section 5]{Lenstra} and \cite[Section 5]{Cadoret2013}. Let $X$ be a connected scheme and consider the category $\mathrm{ECov}(X)$ of finite \'{e}tale coverings $X'\rightarrow{X}$. Let $x:\mathrm{Spec}(\Omega)\rightarrow{X}$ be any geometric point of $X$, where $\Omega$ is an algebraically closed field. If $Y\rightarrow{X}$ is finite \'{e}tale, then so is $Y\times_{X}\mathrm{Spec}(\Omega)$. This gives a functor $\mathrm{ECov}(X)\rightarrow{\mathrm{ECov}(\mathrm{Spec}(\Omega))}$. But the fundamental group of $\mathrm{Spec}(\Omega)$ is trivial, so we obtain an equivalence $\mathrm{ECov}(\mathrm{Spec}(\Omega))\simeq{(\mathrm{Finite}\,\,\mathrm{Sets})}$. This gives the fundamental functor $F_{x}$ for any geometric point $x$. We denote the corresponding profinite group by $\pi(X,x)$.

If $X$ is a normal integral scheme, then there is a very concrete description of $\pi(X,x)$ in terms of the absolute Galois group corresponding to the function field of $X$. Let $K(X)$ be that function field, $\overline{K}$ an algebraic closure of $K(X)$ and consider the composite $M$ of all finite separable extensions $L\subset\overline{K}$ such that the normalization of $X$ in $L$ is finite \'{e}tale over $X$. %$X$ is unramified in $L$. By unramified, we mean that the normalization of $X$ in the field $L$ is unramified over $X$. 
The extension $M/K$ is then Galois and we have an isomorphism $\pi(X,x)\simeq{\mathrm{Gal}(M/K)}$. See \cite[Corollary 6.17]{Lenstra} for the details. %We note that by taking $X:=\mathrm{Spec}(K)$ for some field $K$, we obtain the usual Galois group $\pi(X,x)\simeq{}\mathrm{Gal}(K^{sep}/K)$ where $x:\mathrm{Spec}(K)\rightarrow{\mathrm{Spec}(K)}$ is any morphism. The theory of Galois categories can thus be seen as a generalization of usual Galois theory.  %: \'{e}tale coverings of $\mathrm{Spec}(K)$ correspond to \'{e}tale $K$-algebras which are products of finite separable extensions of $K$.   
\end{exa}

\begin{exa}\label{Grothendieck}
We recall an important result by Grothendieck, which gives a finite representation of the {{tame}} profinite fundamental group of a punctured curve $(X,D)$, where $X$ is now a smooth, proper, connected curve over an algebraically closed field  $k$ of characteristic $p$. %We consider the Galois category of finite \'{e}tale coverings of $(X,D)$ that are tamely ramified. 
 %See \cite[D\'{e}finition 2.1.1]{SGA1} for the definition of the Galois category of finite \'{e}tale coverings that are tamely ramified. 
\begin{theorem}  
Let $(X,D)$ be a smooth proper connected punctured curve over an algebraically closed field $k$ of characteristic $p$ of genus $g:=g(X)$ with $d$ punctures $P_{i}\in{X(K)}$. Then the profinite fundamental group $\pi^{t}(X,D)$ for the Galois category of \'{e}tale coverings of the punctured curve $(X,D)$ that are at most tamely ramified over $D$  is the profinite completion of the group $R=\langle{}x_{i},y_{i},z_{j}\rangle/I$, %for $i=1,..,g$ and $j=1,..,d$, 
where $I$ is the group generated by the single element 
\begin{equation}
\prod_{1\leq{i}\leq{g}}x_{i}y_{i}x_{i}^{-1}y_{i}^{-1}\cdot{}\prod_{1\leq{i}\leq{d}}z_{i}.
\end{equation}
Furthermore, every $z_{i}$ generates an inertia group above the puncture $P_{i}$. 
\end{theorem}
\begin{proof}
See {\normalfont{\cite[Corollaire 2.12]{SGA1}}}\footnote{The theorem in fact holds for separably closed fields $k$. }.
\end{proof}

In other words, the tame profinite fundamental group coincides with the profinite completion of the topological fundamental group of a genus $g$ curve $X/\mathbf{C}$ with $d$ punctures. In fact, the proof of Theorem \ref{Grothendieck} uses this analytic result, along with a theorem on the specialization of the fundamental group.
\end{exa}

\begin{exa}\label{GaloisCategoryResiduallyTame}
{\bf{[Galois-topologically and residually tame coverings]}} Suppose that we fix an algebraic curve $X/K$ with  a set of punctures $D$ as in the beginning of the paper. By Example \ref{ExampleLenstra1}, the category of finite \'{e}tale coverings of $X\backslash{D}$ is a Galois category. We now consider the full subcategory of all finite \'{e}tale coverings of $X\backslash{D}$ whose connected parts are residually (resp. Galois-topologically) tame.  %Galois-topologically tame (resp. residually tame) as in Definition \ref{DefinitionGResTame}. 
We denote these categories by $\mathrm{Cov}_{\mathrm{Tame}}(X,D)$ and $\mathrm{Cov}_{\mathrm{GTop}}(X,D)$.  We will use the induced fundamental functor from the category $\mathrm{ECov}(X,D)$. %We also keep the same fundamental functor. 
Using Lemma \ref{ResiduallyTameLemma} and the fact that $\mathrm{ECov}(X,D)$ is a Galois category, it is then easy to see that these also form a Galois category with profinite fundamental groups equal to $\pi_{\mathrm{Tame}}(X,D)$ and $\pi_{\mathrm{GTop}}(X,D)$. These are the Galois groups of the extensions $M_{\mathrm{Tame}}\supset{K(X)}$ and $M_{\mathrm{GTop}}\supset{K(X)}$ constructed in Lemma \ref{ResiduallyTameLemma}. %Similarly, we can consider the subcategory of all finite \'{e}tale coverings of $X\backslash{D}$ whose connected parts are residually tame. This similarly forms a Galois category with profinite fundamental group $\pi_{\mathrm{GRes}}(X,D)$.   

  % To check the axioms for a Galois category here, we note that the third and fourth follow from the fact that $F$ is a fundamental functor of the Galois category $(F\'{E}tale(X\backslash{D}))$. The second axiom follows by definition. We now check that $(\mathrm{GResTame}(X,D))$ has finite limits and colimits. 

%To check that it has finite limits, it suffices to check that it has fibered products and a final object. $X\backslash{D}$ is again a final object, as in the original case. Let $Z_{i}\rightarrow{X\backslash{D}}$ be two Galois-residually tame coverings. We consider the functor $(\mathrm{GResTame}(X,D))\rightarrow{(\mathrm{F\'{E}tale}(K(X)))}$ by taking the fibered product with $\mathrm{Spec}(K(X))$.  % Then    

% and fibered 

   %We now check that $F$ is a coproduct of connected objects in $(GResTame(X,D))$   

 %We can now use Example \ref{ExampleLenstra1} to conclude that this forms a Galois category as follows.  

% that are analytically tame, as in Definition \ref{AnalyticallyTame}.    %We consider the subcategory of all %now consider the subcategory of the 
\end{exa}

\begin{rem}
Throughout this paper, we will often suppress the base-points in the fundamental functors $F_{x}$ and the profinite fundamental groups $\pi(X,x)$ since they are not of any significant relevance to us.  
\end{rem}






%\begin{exa}\label{Grothendieck}
%We recall an important result by Grothendieck, which gives a finite representation of the {\it{tame}} profinite fundamental group of a punctured curve $(X,D)$, where $X$ is now a smooth, proper, connected curve over a separably closed field $k$ of characteristic $p$. %We consider the Galois category of finite \'{e}tale coverings that are tamely ramified,
% See \cite[D\'{e}finition 2.1.1]{SGA1} for the definition of the Galois category of finite \'{e}tale coverings that are tamely ramified. 
%\begin{theorem}
%Let $(X,D)$ be a smooth proper connected punctured curve over a separably closed field $k$ of characteristic $p$ (we allow $p=0$) of genus $g:=g(X)$ with $d$ punctures $P_{i}\in{X(K)}$. Then the profinite fundamental group $\pi^{t}(X,D)$ corresponding to the Galois category of tamely ramified \'{e}tale coverings of the punctured curve $(X,D)$ is the profinite completion of the group $R=\langle{}x_{i},y_{i},z_{j}\rangle/I$ for $i=1,..,g$ and $j=1,..,d$, where $I$ is the group generated by the single element 
%\begin{equation}
%\prod_{1\leq{i}\leq{g}}x_{i}y_{i}x_{i}^{-1}y_{i}^{-1}\cdot{}\prod_{1\leq{i}\leq{d}}z_{i}.
%\end{equation}
%Furthermore, every $z_{i}$ generates an inertia group above the puncture $P_{i}$. 
%\end{theorem}
%\begin{proof}
%See \cite[Corollaire 2.12]{SGA1}.
%\end{proof}
%In other words, the tame profinite fundamental group coincides with the profinite completion of the fundamental group of any genus $g$ curve $X/\mathbb{C}$ with $d$ punctures. In fact, the proof of Theorem \ref{Grothendieck} uses this analytic result, along with a theorem on the specialization of the fundamental group. % lift the curve $X/k$ to a curve $X/K$ over a field $K$ of characteristic zero and then to use the analytic result.   %uses this analytic fact together with a result on the specialization of the fundamental group
%\end{exa}
 



==> TameSemistableReduction.tex <==
\section{A simultaneous semistable reduction theorem for tame coverings}\label{SectionCoverings}

In this section, we will give a proof of a simultaneous semistable reduction theorem for tame coverings of algebraic curves $\phi:X'\rightarrow{X}$. The theorem seems to be well-known to experts (see \cite[Section 1.2.1]{Cohen2016}), but we included the proof since we couldn't find an exact reference. The theorem will be used to go from the category of finite tame coverings of $(X,D)$ to the category of finite {\it{rigidified}} coverings of any metrized compled $\Sigma(X,D)$ associated to $(X,D)$. This in turn allows us to define the fundamental group of $\Sigma(X,D)$. %define the category of tame coverings of the any skeleton of $X$, which is in turn used to define a tropical fundamental group for a metrized complex of $k$-curves.

The simultaneous semistable reduction theorem for tame coverings we are interested in is as follows:
\begin{theorem}\label{MainThm2}
Let $\phi:X'\rightarrow{X}$ be a finite tame covering of smooth proper connected algebraic curves over $K$ and let $\mathcal{X}$ be any semistable model of $X$ over $R$ such that the closure $\mathcal{B}$ of the branch locus $B\subset{X(K)}$ in $\mathcal{X}$
%\mathcal{B}$ 
consists of disjoint smooth points. %the branch locus reduces to disjoint, smooth points in the special fiber $\mathcal{X}_{s}$. 
Let $\mathcal{X}'$ be the normalization of $\mathcal{X}$ in the function field $K(X')$. Then $\mathcal{X}'$ is semistable and $\mathcal{X}'\rightarrow{\mathcal{X}}$ is a finite morphism of semistable curves over $R$.
\end{theorem}

The earliest versions of this theorem appeared in \cite{liu1} and \cite{liu2}, where it was proved over a discretely valued ring $R$ using techniques of birational geometry and a theorem by Grothendieck on the tame fundamental group of a local Henselian scheme with normal crossings. This theorem was consequently used by the author and Madeline Brandt to give explicit algorithms and descriptions of tropical moduli spaces in \cite{tropabelian} and \cite{supertrop}. The corresponding coverings were referred to as "{\it{disjointly branched coverings}}".

\begin{rem}\label{RemarkEquivalent3}
We note that there are at least two other equivalent ways of formulating the theorem using admissible formal $R$-schemes and Berkovich spaces:
\begin{enumerate}
\item Let $\phi:X'\rightarrow{X}$ and $\mathcal{X}'\rightarrow{\mathcal{X}}$ be as in the theorem and consider the corresponding induced finite morphism of admissible formal $R$ schemes $\mathcal{X}_{\mathrm{form}}'\rightarrow{\mathcal{X}_{\mathrm{form}}}$. Then $\mathcal{X}'_{\mathrm{form}}$ is semistable over $R$ and $\mathcal{X}_{\mathrm{form}}'\rightarrow{\mathcal{X}_{\mathrm{form}}}$ is a finite morphism. %The semistability follows from the equivalence of categories of semistable models over $R$ and semistable formal $R$ models and the finiteness from
This follows from
 \cite[Lemma 5.1 and Theorem 5.13]{ABBR1}. %be a finite tame covering of algebraic curves over $K$, $\mathcal{X}$ a semistable model such that and let $\mathcal{X}$ be any admissible formal $R$-scheme such that the closure of the branch locus reduces to different, smooth points on $\mathcal{X}_{s}$ under the reduction map
%\begin{equation}
%\mathrm{red}:X^{\mathrm{an}}\rightarrow{\mathcal{X}_{s}}.
%%\end{equation}
%Then the normalization $\mathcal{X}'$ of $\mathcal{X}$ is semistable over $R$. %morphism $\mathcal{X}'\rightarrow{\mathcal{X}}$
\item Let $\phi:X'\rightarrow{X}$ be as in the theorem and let $\phi^{\mathrm{an}}:X'^{\mathrm{an}}\rightarrow{X^{\mathrm{an}}}$ be the corresponding analytification in the sense of Berkovich spaces. Let $V$ be a semistable vertex set of $(X,D)$. Then $(\phi^{\mathrm{an}})^{-1}(V)$ is a semistable vertex set of $X'$.
\end{enumerate}
In our proof, we will use the last characterization.
\end{rem}

We will start with some preliminary lemmas. Let $X/K$ and $X'/K$ be two proper, smooth connected curves and let $\phi:X'\rightarrow{X}$ be a finite covering. Then the analytification functor gives a finite morphism $\phi^{\mathrm{an}}:X'^{\mathrm{an}}\rightarrow{X^{\mathrm{an}}}$ on the analytifications by \cite[Proposition 3.4.7]{berkovich2012}. We will denote this morphism by $\phi$ again. For any affinoid domain $U:=\mathcal{M}(A)\subset{X}^{\mathrm{an}}$, we then have $\phi^{-1}(U)=\mathcal{M}(A')$ for some affinoid domain $A'$, and $A'$ is a finite $A$-module. Here we used \cite[3.1.7.(i)]{berkovich2012}. For the upcoming lemma, we will use the following notation. For a $K$-analytic space $Z$, we write $Z^{0}$ for the set of type-$1$ points of $Z$, i.e., 
\begin{equation}
Z^{0}:=\{x\in{Z}:[\mathcal{H}(x):K]<\infty\}.
\end{equation}
\begin{lemma}\label{EtaleLemma}
Suppose that $\phi$ is \'{e}tale above every point of $(X^{\mathrm{an}})^{0}\cap{U}$. Then $\phi$ is \'{e}tale above $U$. %If $\phi^{\mathrm{an}}:\mathcal{M}(B)\rightarrow{\mathcal{M}}$ is \'{e}tale at every closed point
\end{lemma}
\begin{proof}
By \cite[3.3.11]{Berkovich1993}, we have that the morphism of schemes $\mathrm{Spec}(A')\rightarrow{\mathrm{Spec}(A)}$ is \'{e}tale if and only if the morphism $\phi^{-1}(U)\rightarrow{U}$ on the analytifications is \'{e}tale. We will show that $\mathrm{Spec}(A')\rightarrow{\mathrm{Spec}(A)}$ is \'{e}tale. 
Let $M:={\Omega}_{A'/A}$ be the module of K\"{a}hler differentials associated to the homomorphism $A\rightarrow{A'}$. %Then $A\rightarrow{A'}$ is \'{e}tale if and only if ${\Omega}_{A'/A}=(0)$. 
%We write $M$ for this $A'$-module. 
Recall that the maximal ideals of the ring $A'$ correspond bijectively to type $1$ points of $X'^{\mathrm{an}}\cap{\phi^{-1}(U)}$, see \cite[Lemma 2.6.3]{Berkovich1993}. By our assumption, the localization $M_{\mathfrak{m}}$ of $M$ at these points is zero. This implies that $M=0$ by \cite[Chapter 2, Lemma 2.8]{Eisenbud1995}. This proves that $A\rightarrow{A'}$ is unramified by \cite[Chapter 6, Corollary 6.2]{liu2}. Using the fact that $X'$ and $X$ are nonsingular, we quickly obtain flatness using the same localization technique as above. Indeed, $A\rightarrow{A'}$ is flat if and only if $A_{\mathfrak{m}'}$ is flat over every $A_{\mathfrak{m}}$ for every maximal ideal $\mathfrak{m}'$ of $A'$ lying above a maximal ideal $\mathfrak{m}$ of $A$. But these are Dedekind domains, so we obtain flatness by \cite[Chapter 1, Corollary 2.14]{liu2}. We conclude that $\phi$ is flat and unramified, and thus \'{e}tale as desired.%\'{e}tale, as desired.  %This proves that $A\rightarrow{A'}$ is flat, as desired.   
\end{proof}

In other words, if the branch points of $X'\rightarrow{X}$ don't belong to some affinoid domain $U$, then the corresponding covering $\phi^{-1}(U)\rightarrow{U}$ is \'{e}tale. We now recall the following important theorem by Berkovich.
\begin{theorem}\label{BerkovichTheorem2}
{\it{(Tame finite \'{e}tale Galois coverings of open balls and annuli)}}
\begin{enumerate}
\item Let $U$ be an open ball and let $V\rightarrow{U}$ be a finite \'{e}tale Galois covering. Then $V$ is a disjoint union of open balls.
\item Let $U$ be a generalized open annulus, let $V$ be connected and let $V\rightarrow{U}$ be a finite \'{e}tale Galois covering. Then there exist isomorphisms ${\mathbf{S}(a)_{+}}\simeq{U}$ and $V\simeq{\mathbf{S}_{+}(a^{1/n})}$ for $a\in{K}$ such that the composed map is given by $t\mapsto{t^{n}}$. %That is, $\phi$ is {\it{Kummer}}$.  
\end{enumerate}
\end{theorem}
\begin{proof}
The first part is exactly \cite[Theorem 6.3.2]{Berkovich1993}. For the second part, we note that $U$ can be written as a union of closed annuli $\mathbf{S}(a_{1},a_{2})$. To be explicit, let $U\simeq{\mathbf{S}(a)_{+}}$ be an isomorphism for some $a\in{K^{*}}$ and let $c:=\mathrm{val}(a)$. Write $T_{m}=[{c}/{2m},c(1-({1}/{2m}))]$. Then  %We then have that 
\begin{equation}\label{IncreasingUnion}
\mathbf{S}(a)_{+}=\bigcup_{m=1}^{\infty}{\mathrm{trop}^{-1}(T_{m})}.
\end{equation} The induced covering for these closed annuli can then be written as
 \begin{equation}
\mathbf{S}(a_{1}^{1/n},b_{1}^{1/n})\rightarrow{\mathbf{S}(a_{1},b_{1})}
\end{equation}
for some $n$ by \cite[Theorem 6.3.5]{Berkovich1993}. Using Equation (\ref{IncreasingUnion}), %Writing $U$ as an increasing union of closed annuli, 
we then obtain the isomorphism as described in the theorem.  %We note that this $n$ does not change over the various $\mathbf{S}(a,b)$ covering $U$. These isomorphisms then glue together to give a 
\end{proof}

That is, we know what happens to our covering on the $U$ where $\phi$ is \'{e}tale. Let us give an example to illustrate this theorem.
\begin{exa}\label{ExampleCoveringBerkovich}
Let $K:=\mathbf{C}_{p}$ be the field of $p$-adic complex numbers for $p\neq{2}$. Consider the curve $X/\mathbf{C}_{p}$ defined by the affine equation 
$$y^2=x(x-\varpi)(x-\varpi^{2})(x+1)(x+2),$$ where $\mathrm{val}(\varpi)>0$. % is an element of $\mathbb{C}_{p}$ with $v(\pi)>0$. 
The branch points are separated into three groups: 
\begin{align*}
S_{1}&:=\{-1,-2,\infty\}, \\
S_{2}&:=\{\varpi\}, \\
S_{3}&:=\{0,\varpi^{2}\}.
\end{align*}
Consider the closed annuli $V_{1}=\mathbf{S}(\varpi,1)$ and $V_{2}=\mathbf{S}(\varpi^2,\varpi)$ and we let $U_{1}$ and $U_{2}$ be the corresponding open annuli. Let $y_{1}$ and $y_{2}$ and be the type-$2$ points of $V_{1}$ and let $y_{3}$ be the remaining type-$2$ point of $V_{2}$. Here $y_{2}$ is the common type-$2$ point of $V_{1}$ and $V_{2}$. We let $\mathcal{X}$ be the corresponding semistable model, which has three irreducible components in the special fiber. The points of $S_{1}$ reduce to distinct points on the component corresponding to $y_{1}$, $\varpi$ reduces to the component corresponding to $y_{2}$ and the points of $S_{3}$ reduce to distinct points of the third component corresponding to $y_{3}$. For every branch point $P$, we let ${B}_{P}$ be the punctured open ball corresponding to it with respect to $\mathcal{X}$. That is, we have ${B}_{P}=\mathrm{red}_{\mathcal{X}}^{-1}(\tilde{x}_{P})\backslash{\{P\}}$, where $\tilde{x}_{P}$ is the closed point on the special fiber of $\mathcal{X}$ corresponding to $P$.   %and the closed annuli 

The induced coverings of the $U_{i}$ and ${B}_{P}$ of are finite tame and \'{e}tale, with one connected component lying above $U_{1}$ and two components lying above $U_{2}$. %$U_{1}$, $U_{2}$ and $V_{2}$ and two components lying above $V_{1}$.  
The corresponding covering of metrized complexes is given in Figure \ref{Plaatje2}. % \todo{Aanpassen}
\begin{figure}[h!]
\centering
\includegraphics[width=10cm]{{Plaatje2-2.png}}
\caption{\label{Plaatje2} The covering of metrized complexes in Example \ref{ExampleCoveringBerkovich} associated to a hyperelliptic covering $X\rightarrow{\mathbb{P}^{1}}$, where $X$ has genus 2.} %The dual intersection graph for every reduction type as in Theorem \ref{theoremRedType}.}
\end{figure}

Let us give an example of a covering of a closed subannulus of $X^{\mathrm{an}}$ that is not \'{e}tale. Let us take the closed annulus $A'=\tau^{-1}(\Sigma')\subset{X^{\mathrm{an}}}$ where $\Sigma'$ is the closed subset of $\Sigma$ depicted in Figure \ref{Plaatje2} by the blue line. The corresponding induced covering is not \'{e}tale. Indeed, the branch point $\varpi^{2}$ is contained in this annulus. We now easily see from Figure \ref{Plaatje2} that taking a semistable vertex that contains the endpoints of $\Sigma'$ (and not any points in $\Sigma'$) would lead to a vertex set whose complement does not decompose into open annuli and open balls.
   %By considering the open ball ...
%<<Verhaaltje over \'{e}tale ten opzichte van graad overdekking>>%$%B(\pi^{2})$, 
\end{exa}  
We are now ready to prove Theorem \ref{MainThm2}.

\begin{proof}
(Of Theorem \ref{MainThm2}) Let $U$ be a generalized open annulus in $X^{\mathrm{an}}\backslash{V}$. By covering $U$ by affinoid domains and using our assumption on the branch locus, we see from Lemma \ref{EtaleLemma} that $\phi^{-1}(U)\rightarrow{U}$ is \'{e}tale. Let $V\subseteq{U}$ be an affinoid domain with algebra $A$ and let $V'$ be a connected component in $\phi^{-1}(V)$ with corresponding algebra $A'$. We find by \cite[Corollary 3.3.21]{berkovich2012} that $A'$ is an integral domain and we denote its field of fractions by $K(A')$. Taking the Galois closure $L$ of $K(A')\supseteq{K(A)}$ and taking the normalization of $A'$ in $L$, we obtain an finite Galois covering $A''\rightarrow{A}$ which is \'{e}tale. Indeed, by Lemma \ref{EtaleLemma} we can prove this last claim using $K$-rational points. By some basic ramification theory, a covering is \'{e}tale above a $K$-rational point if and only if the Galois closure is \'{e}tale above that point. This proves that the Galois closure is again \'{e}tale.  By Theorem \ref{BerkovichTheorem2}, part two, we now find that $A''\rightarrow{A}$ is Kummer. This then easily implies that the corresponding covering $V'\rightarrow{V}$ is Kummer. Writing $U$ as an increasing union of closed annuli, we thus see that $\phi^{-1}(U)$ is a disjoint union of generalized open annuli, as desired. Similarly, let $U$ be an open ball. As in the previous case, we can reduce to the Galois case and use Theorem \ref{BerkovichTheorem2}, part one, to conclude that $\phi^{-1}(U)$ is a disjoint union of open  balls. 

Now consider all type $2$ points that reduce to type $2$ points in the semistable vertex set $V$. By the previous considerations, we have that the complement consists of generalized open annuli and open balls. This means that it is a skeleton, as desired. 
% \todo{Open ball is geen affinoid, dus veranderen} Let $U=\mathcal{M}(A)$ be an open ball that doesn't contain the branch locus and let $U'$ be a connected component of $\phi^{-1}(U)$ with affinoid $A'$. We extend the induced injection of integral domains $A\rightarrow{A'}$ with quotient fields $K(A)\rightarrow{K(A')}$ to the Galois closure $L$ of the finite extension $K(A')\supset{K(A)}$ and take the normalization $A''$ of $A'$ in this field $L$. By \cite[...]{berkovich2012}, this is an affinoid domain, which is again \'{e}tale over $A$. By Theorem \ref{BerkovichTheorem2} we find that it is trivial, that is, $A''=A'=A$.

%Suppose now that $U=\mathcal{M}(A)$ is a generalized open annulus and let $U'=\mathcal{M}(B)$ be a connected component in $\phi^{-1}(U)$. Note that the covering $U'\rightarrow{U}$ is \'{e}tale.  As in the previous case, we suppose that $\phi^{-1}(U)\rightarrow{U}$ is Galois. Let $\mathbf{S}(b_{1},b_{2})$ be a closed annulus in $A$. The corresponding covering is thus a finite tame \'{e}tale Galois covering and by Theorem \ref{BerkovichTheorem}, we find that the inverse image of $\mathbf{S}(b_{1},b_{2})$ in $A'$ is the annulus $\mathbf{S}(b_{1}^{1/n},b_{2}^{1/n})$ for some $n$. Writing $A$ as a union of closed annuli, we then find that $A'$ is isomorphic to the open annulus $\mathbf{S}(a^{1/n})_{+}$ and the corresponding morphism $\mathbf{S}(a^{1/n})_{+}\simeq{A'}\rightarrow{A}\simeq{\mathbf{S}(a)_{+}}$ is given by $t\mapsto{t^{n}}$. In other words, the covering is Kummer.

%We have now shown that the inverse image of any open ball or generalized annulus is again an open ball or a generalized annulus. This immediately implies that $\phi^{-1}(\Sigma)$ is a skeleton, which gives the Theorem.
 %because it is the product of finitely many \'{e}tale algebras (namely $\sigma(A'')$, where $\sigma\in\mathrm{Gal}(L/K(A))$).  %Extending the morphism $A\rightarrow{A'}$ to the Galois closure
\end{proof}

\begin{exa}\label{EllipticCurveExample1}
We now review Example \ref{ExampleFiberProduct} from the algebraic point of view. Let $E$ be the elliptic curve over $K:=\mathbf{C}_{p}$ defined by the Weierstrass equation
\begin{equation}
y^2=x(x-\varpi)(x+1),
\end{equation}
where $v(\varpi)>0$ and $p\neq{2}$. 
The branch points of the natural hyperelliptic covering $(x,y)\mapsto{x}$ are given by $0$, $\varpi$, $-1$ and $\infty$. A semistable model $\mathcal{X}$ that separates the branch locus is then easily found: we take the blow-up of $\mathbb{P}^{1}_{R}$ along the ideal $I=(x,\varpi)$. In terms of Berkovich spaces, we take the decomposition of $\mathbb{P}^{1,\mathrm{an}}$ into the open annulus $\mathbf{S}(\varpi)_{+}$, four punctured open balls corresponding to the branch points and two type $2$-points (which are the endpoints of $\mathbf{S}(\varpi)_{+}$). Using either an explicit calculation (see Example \ref{TwoTorsionEllipticCurve1}) or a general Kummer criterion for the splitting of edges in abelian extensions as in \cite[Proposition 7.2.1]{tropabelian} and \cite[Proposition 4.1]{supertrop}, we see that the inverse image of this decomposition is then as given in Figure \ref{Plaatje1}. Taking the fiber product of the covering $(x,y)\mapsto{x}$ over itself, we then see that we obtain the diagram of Example \ref{ExampleFiberProduct}.

We will study this elliptic curve $E$ again in Example \ref{TwoTorsionEllipticCurve1}, where the focus will be on the $2$-torsion of $E$ and the various coverings of metrized complexes arising from these points.  %the covering of  %see \cite[...]{tropabelian} for a more general Kummer criterion.% The open annulus then splits into two open annuli by applying the Slope formula and the Kummer criterion for the splitting % find that the open annulus $S(\varpi)_{+}$ splits into two disjoint open annuli
\end{exa}


 %Now let $U$ be an open ball corresponding to a branch point $x\in{X(K)}$. Note that by our assumption on the branch locus, open balls corresponding to different branch points are disjoint. Let $z$ be the unique type $2$ point of $U$ and let the $z_{i}\in\phi^{-1}(U)$ be the type $2$ points lying above $z$. For every    



 



     %By \cite[...]{berkovich2012}, there is an equivalence between the category of finite coverings of a proper scheme $X$ and its analytification. 


